Prosody Modifications for Question-Answering in Voice-Only Settings

Many popular form factors of digital assistants---such as Amazon Echo, Apple Homepod, or Google Home---enable the user to hold a conversation with these systems based only on the speech modality. The lack of a screen presents unique challenges. To satisfy the information need of a user, the presentation of the answer needs to be optimized for such voice-only interactions. In this paper, we propose a task of evaluating the usefulness of audio transformations (i.e., prosodic modifications) for voice-only question answering. We introduce a crowdsourcing setup where we evaluate the quality of our proposed modifications along multiple dimensions corresponding to the informativeness, naturalness, and ability of the user to identify key parts of the answer. We offer a set of prosodic modifications that highlight potentially important parts of the answer using various acoustic cues. Our experiments show that some of these prosodic modifications lead to better comprehension at the expense of only slightly degraded naturalness of the audio.

==> fig-results-emphasis.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=.48\linewidth, valign=t]{figs/emphasis_informativeness.png}
    \includegraphics[width=.48\linewidth, valign=t]{figs/emphasis_correctness.png}
    \caption{Empirical histogram of the \emph{informativeness} ratings (above)
and Gaussian kernel density estimate for \emph{correctness} scores (below) of
the audio with emphasis vs.\ the baseline.
We show density estimate for
the real-valued \emph{correctness} scores to be less affected by
the choice of the bin boundaries, while discrete \emph{informativeness}
ratings have naturally occurring bins. Higher scores are better.}
    \label{fig:emphasis}
\end{figure}

